The Perils of Detecting Measurement Faults in Environmental Monitoring Networks

Scientists deploy environmental monitoring net-works to discover previously unobservable phenomena and quantify subtle spatial and temporal differences in the physical quantities they measure. Our experience, shared by others, has shown that measurements gathered by such networks are perturbed by sensor faults. In response, multiple fault detection techniques have been proposed in the literature. However, in this paper we argue that these techniques may misclassify events (e.g. rain events for soil moisture measurements) as faults, potentially discarding the most interesting measurements. We support this argument by applying two commonly used fault detection techniques on data collected from a soil monitoring network. Our results show that in this case, up to 45% of the event measurements are misclassified as faults. Furthermore, tuning the fault detection algorithms to avoid event misclassification, causes them to miss the majority of actual faults. In addition to exposing the tension between fault and event detection, our findings motivate the need to develop novel fault detection mechanisms which incorporate knowledge of the underlying events and are customized to the sensing modality they monitor.

==> abstract.tex <==
\begin{abstract} 
A number of recent studies have reported the
prevalence of sensor faults. This work investigates the detection of
these faults using commonly employed fault detection techniques in the
presence of events.  We apply these techniques to data collected from
a real deployment containing events. In particular, we focus our
efforts on box temperature and soil moisture: two commonly observed
modalities. We find that due to certain statistical properties of
events, they are often misclassified as faults, which can harm certain
types of environmental monitoring applications. We investigate reasons
and conditions which lead to this misclassification and argue that
event signatures need to be leveraged to disambiguate events and
faults.  . The main contribution of this paper is to bring forward the
duality that exists between events and faults and to discuss the
implications of the robustness properties that is desired from the
fault detection scheme.

%the similarities and differences involved in 
%detecting events and sensor faults in environmental monitoring 
%applications of sensor networks. Event detection and fault 
%detection are both important in their own right. We draw a connection
%between detecting faults and events and argue that fault detection
%schemes must not mis-classify events as faults, leading to the loss
%of valuable information. We study some commonly applied fault detection
%techniques and characterize their misclassification error. These techniques
%are applied to data obtained from a real soil monitoring deployment 
%having multiple modalities. We find that events are often misclassified
%as faults due to similarities in their statistical properties to faults.
%In our implication section, we suggest ways to handle this problem and
%address some of the issues related with the solution.
\end{abstract}


==> ack.tex <==
\section*{Acknowledgments}
\label{sec:ack}
Acknowledgements here ..


==> intro.tex <==
\section{Introduction}
\label{sec:intro}

Wireless Sensor networks have facilitated spatial and temporal data
collection at rates which were previously unimaginable.  A number of
testbeds ~\cite{SSC+06}, ~\cite{FFCENS06} have demonstrated that the
data obtained from these deployments is inherently noisy and full of
faults. This has led the community to investigate various aspects
related to detecting sensor faults. Detecting faults can significantly
cut down on communication and storage costs.  A problem which is very
closely related to fault detection is one of ``event detection''. An
event can be defined as a period of ``interesting'' activity. The
definition of an event may vary depending on the type of
application. For example, in a soil monitoring application,
precipitation can be regarded as an event, and for the rest of the
paper, we will use the meaning of an event in this context. For
scientists, these event periods represent periods of change and
transition, and provide valuable insight into the phenomenon being
observed. Thus, scientists would want the application to collect more
information during these periods compared to more predictable
periods. These events reflect sharp transient changes in the sensing
modalities and can often be misclassified as faults. In fact, it is
very important to detect these events so that one can switch to a
higher sampling frequency to collect more data.  One could argue that
faults are a special case of events. However, we find that despite
having certain similarities, rain events and faults have prominent
differences in statistical characteristics, which should be leveraged
for classification.  An interesting aspect of the interplay between
detecting events and faults is the action taken after detecting
them. Faulty data points must be thrown away (or repaired) if the
sensor is found to be faulty.  On the other hand, the detection of an
event might cause one to switch to a higher sampling frequency.  As
far as we know, no one has looked at fault detection from this light
and this is the first step in this direction.


This paper does not address detection of events, but instead, focusses
at understanding the misclassification of events as faults by some
commonly employed fault detection techniques.  In section
\ref{sec:sol} we describe commonly occurring, well known faults that
are used in this work, their description, and techniques which are
meant to detect these faults.  Section \ref{sec:res} describes the
evaluation metrics used by us to study this
misclassification. Furthermore, we describe the method of injecting
faults, giving us fault ground truth . We close the section by
presenting our results and providing intuition on those numbers.
Finally, we conclude the paper in Section \ref{sec:imply} by providing
an account of the implication of these results and bringing up some
relevant discussion issues.


Fault detection has gathered considerable momentum in the sensor
community over the past few years. The theme behind this line of
questioning is to bridge the gap between events and faults and bring
to the table that events are an important aspect of environmental
monitoring and need to be dealt with care and caution.  As per our
knowledge, events have never been looked under the fault
microscope. In this paper, we demonstrate that fault detection
techniques are vulnerable to this misclassification and argue that
certain applications require techniques that need to be robust in the
presence of events.  We stress the importance of signatures exhibited
by different modalities on events and argue that they play a pivotal
role in reducing this miclassification. Our evaluation metrics are
unique and could be a crucial component in the choice of the fault
detection technique that should be used for the application. Finally,
we stress the duality of events and faults and point out that the
system design should consider their trade-off.


\subsection{Event Signatures in Environment monitoring}

Data from different modalities in an environmental monitoring
application often has different characteristics. Moreover, these
characteristics will manifest themselves differently during
events. For example, box temperature and soil moisture are two
commonly sensed modalities in a typical environmental monitoring
application.  Figure \ref{fig:sig} shows a motivating example of the
typical reactions shown by box temperature and soil moisture
modalities to a rain event. The figure shows a non-event day followed
by a day which sees considerable rain. One can notice the change in
the box temperature signal from the mean signal on the event day as
compared to the non-event day, which conforms well to the expected
behaviour.  In contrast to box temperature, soil moisture reacts very
differently.  The onset of the event causes a sudden jump in the value
recorded by the soil moisture sensor followed by a period of slow
decay. The amount of rainfall and the event duration are some of the
factors that influence the nature of the reaction.



\begin{figure}[t]
\begin{center}
  \epsfig{file=plots/event_signature.eps, width=0.9\columnwidth} \\
  \caption {Reaction of the box temperature and soil moisture
  modalities to a rain event.}  
\label{fig:sig}
\end{center}
  \end{figure}

%etc
%For example, consider a situation
%where the user is interested in knowing the average value across all
%sensors in a given sensing environment in the presence of sensor
%faults.  Faulty sensor readings would not only pollute the statistic,
%but also waste a lot of power by transmitting faulty readings to the
%unit undertaking the computation.  Over the past couple of years, a
%number of groups have been working on addressing issues linked with
%fault detection right from classifying the type of sensor faults to
%providing methods to detect these faults.
%



==> results.tex <==
\section{Evaluation}
\label{sec:res}

%We begin by establishing metrics to study the misclassification of
%events as faults. We describe our data and the process of injecting
%faults into our test data, creating an evaluation set which contains
%events and faults. Last but not least, we describe our
%results and provide some intuition on their interpretation.


\subsection {Evaluation Metrics}
\label{sec:metric}

In order to study the misclassification of events as faults, we need
to establish appropriate metrics. The misclassification metric we use
has two variants depending on the method under evaluation. First, the
SHORT-rule and the LLSE methods classify individual sensor readings as
faulty and therefore the misclassification error $\mu$ can be defined
as $$
\mu = 
\frac{\textrm{number of event measurements tagged as
faults}}{\textrm{total number of event measurements}}  
$$ 
In this case, an \emph{event measurement} is a sensor reading
(\emph{e.g.} box temperature) during an event (rainfall). 

On the other hand, the NOISE-rule method declares sets of $N$
successive samples as faulty and therefore the metric must account for
the misclassification duration. Let us say that the duration of the
$i$-th event is $E_i$ and let $F_i$ be the time during which a set of
successive samples are declared to be faulty. Then, all periods $D_i$
within $F_i$ that overlap with $E_i$ contribute to the
misclassification error. One can then obtain the total
misclassification error by summing over all time periods of
misclassification: $$
\mu = \frac {\sum_{i} D_i}{\sum_{i} E_i}
$$
	
Having established a misclassification metric, we need a metric to
study the efficacy of the fault detection method itself. The reason is
that one can set a method's parameters to minimize the number of
misclassifications. Doing so however, might cause the method to fail
to detect the actual faults. We use the false negative ratio, defined
as the fraction of faults that were not detected by the method to the
total number of faults, for this purpose.

\subsection{Data}

We apply the fault detection techniques presented in
Section~\ref{sec:method} to the data obtained from the Jug bay turtle
monitoring sensing network ~\cite{AGU07}. Specifically, we use the box
temperature and soil water content (\emph{i.e.}, soil moisture)
modalities collected by three motes at the deployment site. The raw
data series uses ten minute intervals but we derive a more smooth data
series by calculating the average of every two sensor readings.


Approximately five months of data were collected from the Jug bay
sensor deployment, from 2007/06/22 to 2007/11/27.  We use one month of
data from each of the sensors for training purposes and the rest as
test data.  The training data was thoroughly cleaned using a median
filter.  Moreover, we visualized the data and manually removed any
faulty readings to make the training set devoid of faults. The set of
events that occurred during the deployment period is gathered from a
weather station located one kilometer away from the monitoring site,
which records precipitation data at 15-minute intervals~\cite{JBPR}.
Twenty one major events occurred during the measurement period,
spanning a total of 9,480 rainfall minutes (158 hours).

\subsection{Fault Injection}

As we mentioned in Section~\ref{sec:metric}, we are also interested in
the percentage of real faults that the detection algorithms
miss. However, in order to calculate this ratio we need to know which
measurements correspond to actual faults. Considering that we have no
way of knowing which actual sensor readings are faulty, we resort to
artificially injecting SHORT and NOISE faults. To do so, we use the
procedure outlined by Sharma et al.~\cite{SECON07}.

To inject a SHORT fault, a sample $v_i$ is picked at random and is
replaced by the value $\hat{v_i} = v_i + f*v_i$.  SHORT faults with
intensities $f = \{0.5,1,2\}$ and $f = \{0.1,0.2,0.5\}$ were injected
in the test set for box temperature and soil moisture respectively.
To inject a NOISE fault, a set of $W$ successive samples is randomly
chosen and random values drawn from the distribution $\sim N(0,
\sigma^2)$ are added to the test set.  NOISE faults causing an increase
of $0.5\times, 1.5 \times,$ and $3 \times$ in standard deviation ($\sigma$)
were injected in the box temperature and soil moisture test data sets.


The fraction of SHORT faults in the data was set at $1.5\%$, while the
fraction of NOISE fault samples was set at $6.5\%$. Finally, we set
the the value of $W$ to have $|W|/N$ equal to 3/2 for both box
temperature and soil moisture. Note that SHORT faults are ephemeral
and are thus are much more in number compared to the NOISE faults
which last for longer periods of time. Figure~\ref{fig:BTfaults}
provides an example of the artificially injected fault data for box
temperature. 

\begin{figure}[t]
\begin{center}
  \epsfig{file=plots/BoxTempFaults.eps, width=\columnwidth} \\
  \caption {Box temperature test data after injecting SHORT and NOISE
faults.}  
\label{fig:BTfaults}
\end{center}
\end{figure}




\subsection{Results}






%\begin{figure}[t]
%\begin{center}
%  \epsfig{file=plots/BT_SHORT.eps, width=0.9\columnwidth} \\
%  \caption {Misclassification of events as SHORT faults for
%  box temperature as a function of the $\delta$ threshold. Also shown is
%the percentage of false negatives.}  
%\label{fig:bt_sht}
%\end{center}
%  \end{figure}
%

In order to detect SHORT faults in box temperature data, we vary the
SHORT threshold ($\delta$) from $10^\circ C$ to $60^\circ C$ in
increments of $5^\circ C$. Figure~\ref{fig:bt_sht} plots the
misclassification error and the percentage of false negatives for box
temperature as a function of increasing $\delta$. We observe that low
values of $\delta$ result in low false negative ratios but also suffer
from high misclassification errors. On the other hand, increasing
$\delta$, reduces the misclassification error at the expense of
failing to detect the majority of the faults. 

Figure~\ref{fig:sm_sht} shows the effect of varying $\delta$ for soil
moisture data.  At low values of $\delta$, even though the percentage
of false negatives is low, the misclassification error is as high as
64\%. This result is not surprising for the soil moisture modality
because during the onset of an event the soil moisture sensor shows a
sharp change which resembles a SHORT fault. The misclassification
error is much lower in the case of box temperatures because they do
not show sharp leading edge behaviors during an event's onset.

  
%\begin{figure}[t]
%\begin{center}
%  \epsfig{file=plots/SM_SHORT.eps, width=0.9\columnwidth} \\
%  \caption {Misclassification of events as SHORT faults for
%  soil moisture as a function of the $\delta$ threshold. Also shown is
%the percentage of false negatives.}  
%\label{fig:sm_sht}
%\end{center}
%  \end{figure}
%

The NOISE-rule operates on a window of $N$ consecutive samples. We
study the misclassification error as a function of
$\sigma_{allow}$. Figure~\ref{fig:bt_nse} shows that at low values of
$\sigma_{allow}$ the misclassification error is high. It is
interesting to note that the false negative percentage does not vary
at all for $\sigma_{allow} \in \{1,1.5,2,2.5\}$ in spite of the
dropping misclassification error. This behavior can be explained by
the observation that box temperature tends to drop during, before, and
after a rain event. Thus the misclassification is caused on the lower
side of the rule $(\sigma_{NOISE} - \sigma_{allow})$.  We performed
similar analysis on the soil moisture data. However, because soil
moisture values do not change by much, unless reacting to events, the
resulting misclassification error was not sensitive to the value of
$\sigma_{NOISE}$.


%\begin{figure}[t]
%\begin{center}
%  \epsfig{file=plots/BT_NOISE.eps, width=0.9\columnwidth} \\
%  \caption {Misclassification of events as NOISE faults for
%  box temperature as a function of $\sigma_{allow}$. Also shown is
%the percentage of false negatives.}  
%\label{fig:bt_nse}
%\end{center}
%  \end{figure}
%

For the LLSE method, we set $p$ to 95\% and $q$ to two. Table
\ref{tab:llse} presents our findings for the two sensing modalities we
used. The higher misclassification error associated with soil moisture
is expected. This is because soil moisture sensors react differently
depending on their location. Figure~\ref{fig:reaction} presents an
example of this phenomenon, by plotting the reaction of three soil
moisture sensors to a rain event. Node 5 and Node 6 tend to move
together, whereas the reaction of Node 2 is much lower in magnitude.

%\begin{figure*}[t]
%\begin{center}
%  \begin{tabular}{c | c}
%  \epsfig{file=plots/SM_SHORT.eps, width=0.5\linewidth, clip=} 
%   & \epsfig{file=plots/BT_SHORT.eps, width=0.5\linewidth, clip=} \\ 
%  \epsfig{file=plots/SM_NOISE.eps, width=0.5\linewidth, clip=} 
%   & \epsfig{file=plots/BT_NOISE.eps, width=0.5\linewidth, clip=} \\ 
%  \end{tabular}
%  \caption {The left panel shows the misclassification of SHORT faults (top)
%  and NOISE faults (bottom) for soil moisture. The right panel shows the
%  misclassification of SHORT faults (top) and NOISE faults (bottom) for
%  box temperature}
%  \label{fig:mis}
%\end{center}
%  \end{figure*}


\begin{figure*}[ht!]
	\centering
	\setcounter{subfigure}{0}
	\subfigure[Soil Moisture SHORT-rule ]{
		\label{sfig:sm_short}\includegraphics[width=0.45\linewidth]{plots/SM_SHORT.eps}
	}\,
	\setcounter{subfigure}{1}
	\subfigure[Box Temperature SHORT-rule]{
		\label{sfig:bt_short}\includegraphics[width=0.45\linewidth]{plots/BT_SHORT.eps}
	}\\
	\setcounter{subfigure}{2}
	\subfigure[Soil Moisture NOISE-rule]{
		\label{sfig:sm_noise}\includegraphics[width=0.45\linewidth]{plots/SM_NOISE.eps}
	}\,
	\setcounter{subfigure}{3}
	\subfigure[Box Temperature NOISE-rule]{
		\label{sfig:bt_noise}\includegraphics[width=0.45\linewidth]{plots/BT_NOISE.eps}
	}\\

	\caption{{\bf Results:} 
	The misclassification error and fault negative fractions for 
	the soil moisture and box temperature modalities using the SHORT and NOISE rule.
	(a) also shows the misclassification error in the first half hour
	of events caused due to the reaction of soil moisture 
	on the onset of an event.
	}
\end{figure*}




\begin{figure}[t]
\begin{center}
  \epsfig{file=plots/swp_reaction.eps, width=0.9\columnwidth} \\
  \caption {Reactions of different soil moisture
  sensors to a rain event.}  
\label{fig:reaction}
\end{center}
\end{figure}


\begin{table} [t]
\caption{Misclassification error for the LLSE method} 
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Modality  &  Misclassification & False \\
 & error & Negatives \\
\hline 
Box Temperature & 0.3\% & 77.19\% \\
\hline 
Soil Moisture & 46.3\% & 50.03\% \\
\hline
\end{tabular}
\label{tab:llse}
\end{center}
\end{table}





